Empirical Characterization of Logging Smells in Machine Learning Code

Logging plays a central role in ensuring reproducibility, observability, and reliability in machine learning (ML) systems. While logging is generally considered a good engineering practice, poorly designed logging can negatively affect experiment tracking, security, debugging, and system performance. In this paper, we present an empirical study of logging smells in ML projects and propose a taxonomy of ML-specific logging smell types. We conducted a large-scale analysis of 444 ML repositories and manually labeled 2,448 instances of logging smells. Based on this analysis, we identified 12 categories of logging smells spanning security, metric management, configuration, verbosity, and context-related issues. Our results show that logging smells are widespread in ML systems and vary in frequency and manifestation across projects. To assess practical relevance, we conducted a survey with 27 ML practitioners. Most respondents agreed with the identified smells and reported that several types, including Logging Sensitive Data, Metric Overwrite, Missing Hyperparameter Logging, and Log Without Context, have a strong impact on reproducibility, maintainability, and trustworthiness. Other smells, such as Heavy Data Logging and Print-based Logging, were perceived as more context-dependent. We publicly release our labeled dataset to support future research. Our findings highlight logging quality as a critical and underexplored aspect of ML system engineering and open opportunities for automated detection and repair of logging issues.

==> 0_Preamble.tex <==
% First comes an example EPS file -- just ignore it and
% proceed on the \documentclass line
% your LaTeX will extract the file if required
% \begin{filecontents*}{example.eps}

% %%BoundingBox: 19 19 221 221
% %%CreationDate: Mon Sep 29 1997
% %%Creator: programmed by hand (JK)
% %%EndComments
% gsave
% newpath
%   20 20 moveto
%   20 220 lineto
%   220 220 lineto
%   220 20 lineto
% closepath
% 2 setlinewidth
% gsave
%   .4 setgray fill
% grestore
% stroke
% grestore
% \end{filecontents*}
%
\RequirePackage{fix-cm}

% Need To Remove Before Submit
\AtBeginDocument{%
  \paperwidth=\dimexpr
    1in + \oddsidemargin
    + \textwidth
    % + \marginparsep + \marginparwidth
    + 1in + \oddsidemargin
  \relax
  \paperheight=\dimexpr
    1in + \topmargin
    + \headheight + \headsep
    + \textheight
    % + \footskip
    + 1in + \topmargin
  \relax
  \usepackage[pass]{geometry}\relax
}
% ---------------------------------------------------------------------------------------------------------------------------
% \setcounter{tocdepth}{3}
% \setcounter{secnumdepth}{3}
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{soul}	
\usepackage{balance}
\usepackage{tabularx}
\usepackage{enumitem}
\usepackage{adjustbox}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{caption}
% \usepackage{hyperref}
\usepackage{dirtytalk} 
\usepackage{xcolor}
\usepackage[most]{tcolorbox}
\usepackage{pifont}
\usepackage[mathlines,switch]{lineno}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{%
            \node[shape=circle,draw,inner sep=1pt] (char) {#1};}}
\usepackage{tikz}
% \setlength{\parindent}{15pt}  % Set paragraph indentation
% \setlength{\parskip}{0pt}     % Disable extra space between paragraphs
% ---------------------------------------------------------------------------------------------------------------------------
%
\usepackage{graphicx}
\usepackage{listings}
% \usepackage{color}
\usepackage{pifont}
\usepackage{amsmath}
\usepackage{pdflscape} 
\usepackage{tikz}
\usepackage{dirtytalk}
\usepackage{makecell}
\usepackage[title]{appendix}
\usepackage{pythonhighlight}
%\usepackage[newfloat]{minted}
\usepackage{caption}
\newenvironment{code}{\captionsetup{type=listing}}{}
%\SetupFloatingEnvironment{listing}{name=Source Code}
% \usepackage{xcolor} % to access the named colour LightGray
\definecolor{LightGray}{gray}{0.9}
%\usepackage{minted}
% \setcounter{tocdepth}{3}
% \setcounter{secnumdepth}{3}

\usepackage[autostyle]{csquotes}
\usepackage{longtable}
\usepackage{booktabs}
\usepackage{tablefootnote}
\usepackage{multirow}
\usepackage{adjustbox}
\usepackage{enumitem}
\usepackage{siunitx}
\usepackage{fancyvrb}
\usepackage{soul}
\usepackage{textcomp}
\usepackage{tabularx}
\usepackage[utf8]{inputenc}   % For modern UTF-8 input (not needed with pdflatex + lualatex)
% \usepackage{textcomp}         % Adds additional symbols like \textquotedbl, \textquotesingle, etc.
\newlength\someheight
\setlength\someheight{3cm}
\lstset{upquote=true}
\usepackage[T1]{fontenc}     % Switch to T1 font encoding (supports \textquotedbl)
\usepackage{textcomp}        % Enables \textquotedbl and related symbols
\usepackage{listings}
\lstset{upquote=true}        % Ensures correct display of straight quotes in code

\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=1.14}
\definecolor{storeClusterComponent}{HTML}{808080}
\definecolor{dbscan}{HTML}{BEBEBE}
\definecolor{constructCluster}{HTML}{DCDCDC}
\usepackage{tikz} 
\usepackage{subcaption}
% \usetikzlibrary{shapes.geometric}
\usetikzlibrary{shapes,calc,shadows,arrows}
\usepackage{pgf-pie}
\usepackage{etoolbox}
\newtoggle{showpct}
\usepackage{xcolor,colortbl}
% \usepackage{indentfirst}
% \setlength{\parindent}{15pt}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

% Define Python-specific settings for listings
% \lstdefinestyle{python}{
%     language=Python,
%     basicstyle=\ttfamily\tiny,
%     keywordstyle=\color{blue}\bfseries,
%     commentstyle=\color{green!50!black}\itshape,
%     stringstyle=\color{red},
%     showstringspaces=false,
%     frame=single,
%     numbers=left,
%     numberstyle=\tiny\color{gray},
%     stepnumber=1,
%     numbersep=5pt,
%     breaklines=true,
%     breakatwhitespace=true,
%     tabsize=4,
%     captionpos=b
% }

\lstdefinestyle{python}{
    language=Python,
    backgroundcolor=\color{backcolour}, 
    basicstyle=\tiny,         % Smaller than \tiny for better readability
    keywordstyle=\color{blue},
    commentstyle=\color{green!50!black},
    stringstyle=\color{red},
    showstringspaces=false,
    frame=single,
    numbers=left,
    upquote=true,
    numberstyle=\tiny\color{gray},
    stepnumber=1,
    numbersep=3pt,                            % Tighter margin between code and line numbers
    breaklines=true,
    breakatwhitespace=true,
    tabsize=1,                                % Smaller tab size for compact indentation
    captionpos=b,
    aboveskip=2pt,                            % Reduce spacing before listing
    belowskip=2pt                             % Reduce spacing after listing
}


% Default style for listings
\lstset{style=python}

% \lstdefinestyle{mystyle}{
%     backgroundcolor=\color{backcolour},   
%     commentstyle=\color{codegreen},
%     keywordstyle=\color{magenta},
%     numberstyle=\tiny\color{codegray},
%     stringstyle=\color{codepurple},
%     basicstyle=\ttfamily\footnotesize,
%     breakatwhitespace=false,         
%     breaklines=true,                 
%     captionpos=b,                    
%     keepspaces=true,                 
%     numbers=left,                    
%     numbersep=5pt,                  
%     showspaces=false,                
%     showstringspaces=false,
%     showtabs=false,                  
%     tabsize=2
% }
\usepackage[most]{tcolorbox}
%\usepackage{minted}

\newtcbtheorem{Summary}{\bfseries Summary}{enhanced,drop shadow={black!50!white},
  coltitle=black,
  top=0.3in,
  attach boxed title to top left=
  {xshift=1.5em,yshift=-\tcboxedtitleheight/2},
  boxed title style={size=small,colback=pink}
}{summary}


\newtcolorbox[auto counter]{summary}[1][]{title={\bfseries Summary~\thetcbcounter},enhanced,drop shadow={black!50!white},
  coltitle=black,
  top=0.3in,
  attach boxed title to top left=
  {xshift=1.5em,yshift=-\tcboxedtitleheight/2},
  boxed title style={size=small,colback=pink},#1}

\usepackage[round]{natbib}


\usepackage{etoolbox}
% \usepackage[hyphens]{url}
% \usepackage{hyperref}
% \PassOptionsToPackage{hyphens}{url}
% \hypersetup{colorlinks,
%     citecolor=blue, 
%     urlcolor=black,
%     linkcolor=blue}
% \newcommand*{\escape}[1]{\texttt{\textbackslash#1}}
% \newcommand*\circled[1]{\tikz[baseline=(char.base)]{
%             \node[shape=circle,draw,inner sep=1pt] (char) {#1};}}
\makeatletter
\patchcmd{\pgfpie@slice}%
{\scalefont{#3}\beforenumber#3\afternumber}%
{\iftoggle{showpct}{\scalefont{#3}\beforenumber#3\afternumber}{}}%
{}{}

% Patch case where name and year are separated by aysep
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}

% Patch case where name and year are separated by opening bracket
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
       {\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
  {}{}

\def\srcfile[#1,#2]#3{
    \node [draw, fill=white, minimum height=1.7cm, minimum width=1.35cm, rounded corners, double copy shadow={shadow xshift=0.1cm, shadow yshift=0.1cm}] (#1) at #2 {};
    \node[align=center, font=\sffamily\fontsize{5}{1.5}\selectfont] at #2 {#3};
}

\makeatother

\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}
\definecolor{dgreen}{rgb}{0.0, 0.5, 0.0}

%\renewcommand{\lstlistingname}{Figure}
\lstset{
    frame=single,
    tabsize=4,
    showstringspaces=false,
    columns=flexible,
    basicstyle={\small\ttfamily},
    keywordstyle=\color{blue},
    commentstyle=\color{dkgreen},
    stringstyle=\color{mauve},
    breaklines=true,
    breakatwhitespace=true,
    escapeinside={<@}{@>},
}

\usepackage{mdframed}
\newcounter{finding}
\newmdenv[%
    linewidth=0.6pt,
    linecolor=black,
    outerlinewidth=0pt,
    skipabove=0pt,
    skipbelow=0pt,
    settings={\global\refstepcounter{finding}},
]{myfinding}

\newcommand{\finding}[1]{
    \vspace{0.5em}
    \begin{myfinding}
    % \vspace{0.25em}
	\textbf{\textit{Finding~\arabic{finding}}}: #1
 	% \vspace{-0.25em}
    \end{myfinding}
    \vspace{0.5em}
}


\newcommand{\yiming}[1]{\textcolor{violet}{{\it [Yiming says: #1]}}}
\newcommand{\haonan}[1]{\textcolor{dkgreen}{{\it [Haonan says: #1]}}}
\newcommand{\maxime}[1]{\textcolor{red}{{\it [Max says: #1]}}}
\newcommand{\heng}[1]{\textcolor{blue}{{\it [Heng says: #1]}}}

\newcommand{\hadoop}{\href{https://github.com/apache/hadoop}{\javainline{Hadoop}}}
\newcommand{\hadoopO}{\href{http://hadoop.apache.org}{\javainline{Hadoop}}}
\newcommand{\jboss}{\href{http://www.jboss.org/jbossas}{\javainline{JBoss}}}
\newcommand{\hbase}{\href{https://github.com/apache/hbase}{\javainline{Hbase}}}
\newcommand{\hive}{\href{https://github.com/apache/hive}{\javainline{Hive}}}
\newcommand{\zookeeper}{\href{https://github.com/apache/zookeeper}{\javainline{Zookeeper}}}
\newcommand{\tomcat}{\href{https://github.com/apache/tomcat}{\javainline{Tomcat}}}
\newcommand{\lucene}{\href{https://github.com/apache/lucene-solr}{\javainline{Lucene-solr}}}
\newcommand{\actvieMQ}{\href{https://github.com/apache/activemq}{\javainline{ActiveMQ}}}
\newcommand{\maven}{\href{https://github.com/apache/maven}{\javainline{Maven}}}
\newcommand{\ant}{\href{https://github.com/apache/ant}{\javainline{Ant}}}
\newcommand{\empireDB}{\href{https://github.com/apache/empire-db}{\javainline{Empire-DB}}}
\newcommand{\karaf}{\href{https://github.com/apache/karaf}{\javainline{Karaf}}}
\newcommand{\logfj}{\href{https://github.com/apache/log4j}{\javainline{Log4j}}}
\newcommand{\mahout}{\href{https://github.com/apache/mahout}{\javainline{Mahout}}}
\newcommand{\mina}{\href{https://github.com/apache/mina}{\javainline{Mina}}}
\newcommand{\pig}{\href{https://github.com/apache/pig}{\javainline{Pig}}}
\newcommand{\pivot}{\href{https://github.com/apache/pivot}{\javainline{Pivot}}}
\newcommand{\struts}{\href{https://github.com/apache/struts}{\javainline{Struts}}}
\newcommand{\openmts}{\href{https://github.com/apache/openmeetings}{\javainline{Openmeetings}}}
\newcommand{\fop}{\href{https://github.com/apache/xmlgraphics-fop}{\javainline{Fop}}}
\newcommand{\jmeter}{\href{https://github.com/apache/jmeter}{\javainline{Jmeter}}}
\newcommand{\rat}{\href{https://github.com/apache/creadur-rat}{\javainline{Rat}}}
\newcommand{\gitpython}{\href{https://github.com/gitpython-developers/gitpython}{\javainline{GitPython}}}
\newcommand{\srcML}{\href{https://www.srcml.org/}{\javainline{srcML}}}

%Command to strikeout text with citations and references
\newcommand{\strikeit}[1]{%
  \ifcorrectingmode
  \mbox{\sout{#1}}%
%  \makebox[\textwidth][s]{\sout{#1}}%
  \fi
}

%********** Minted **********
\makeatletter
\newcommand\notsotiny{\@setfontsize\notsotiny\@vipt\@viipt}
\makeatother

\usepackage[draft=false]{minted}
\newminted{diff}{
    % numbersep=4pt,
    % linenos,
    fontsize=\scriptsize,
	autogobble=true,
	% style=bw,
% 	breaklines=true,
% 	breakafter=.,
% 	breakautoindent,
%     tabsize=2,
%     breakbytoken=true,
%     resetmargins=true
}
\newmintinline{cpp}{}
\newminted{python}{}
\newmintinline{python}{}
% \newminted{java}{}
% \newmintinline{java}{}
%%%%%%%%%%%%%%% java in stream
\newminted{java}{
	fontsize=\small,
	autogobble=true,
	% style=bw,
	breaklines=true,
	breakafter=.,
	breakautoindent,
    tabsize=2,
    % linenos=true,
    breakbytoken=true,
    resetmargins=true}
\newmintinline{java}{
	% style=bw,
    fontsize=\small}
\setminted{%
    style=trac,
    autogobble=true,
    breaklines=true,
    breakafter=.,
    breakautoindent,
    escapeinside=||}
\newcommand{\textjavainline}[1]{\ensuremath\text{\javainline{#1}}}
\DeclareCaptionSubType{listing}
\newcommand{\ji}[1]{\javainline{#1}}

\let\proof\relax
\let\endproof\relax
\let\example\relax
\let\endexample\relax
\usepackage{amsthm}

\theoremstyle{definition}
\newtheorem{dfn}{Definition}

\usepackage{threeparttable}

\usepackage{array}
\definecolor{dodgerblue}{RGB}{30,144,255}
\definecolor{orange}{RGB}{255, 120, 8}

\newcommand{\lstbg}[3][0pt]{{\fboxsep#1\colorbox{#2}{\strut #3}}}
\lstdefinelanguage{diff}{
  basicstyle=\ttfamily\small,
  morecomment=[f][\lstbg{red!20}]-,
  morecomment=[f][\lstbg{green!20}]+,
  morecomment=[f][\textit]{@@},
  %morecomment=[f][\textit]{---},
  %morecomment=[f][\textit]{+++},
}

\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}

% \usepackage[skins]{tcolorbox}
\tcbset{commonstyle/.style={boxrule=0pt,sharp corners,enhanced jigsaw,nobeforeafter,boxsep=0pt,left=\fboxsep,right=\fboxsep}}
\newtcolorbox{mycolorbox}[1][]{commonstyle,#1}

\newcommand{\wrapcolorbox}[2][]{%
  \colorbox{#1}{\tiny \parbox{\dimexpr\linewidth-2\fboxsep}{#2}}
}

\newcommand{\responsecolorbox}[2][]{%
  \colorbox{#1}{\small \textit{\parbox{\dimexpr\linewidth-2\fboxsep}{#2}}}
}

\newcommand{\findcolorbox}[2][]{%
  \vspace{-0.15cm}
  \colorbox{#1}{\normalsize \parbox{\dimexpr\linewidth-2\fboxsep}{#2}}
%   \vspace{0.1cm}
}

% \newcommand{\inlinecode}[2]{\lstinline[language=#1]$#2$}
\def\inline{\lstinline[basicstyle=\ttfamily \scriptsize]}


\usepackage{svg}


% patch \maketitle:
\usepackage{etoolbox}
\newcommand*{\affaddr}[1]{#1} % No op here. Customize it for different styles.
\newcommand*{\affmark}[1][*]{\textsuperscript{#1}}

% \usepackage[misc]{ifsym}

\usepackage{scalerel}
\usepackage{tikz}
\usetikzlibrary{svg.path}

\definecolor{orcidlogocol}{HTML}{A6CE39}
\tikzset{
  orcidlogo/.pic={
    \fill[orcidlogocol] svg{M256,128c0,70.7-57.3,128-128,128C57.3,256,0,198.7,0,128C0,57.3,57.3,0,128,0C198.7,0,256,57.3,256,128z};
    \fill[white] svg{M86.3,186.2H70.9V79.1h15.4v48.4V186.2z}
                 svg{M108.9,79.1h41.6c39.6,0,57,28.3,57,53.6c0,27.5-21.5,53.6-56.8,53.6h-41.8V79.1z M124.3,172.4h24.5c34.9,0,42.9-26.5,42.9-39.7c0-21.5-13.7-39.7-43.7-39.7h-23.7V172.4z}
                 svg{M88.7,56.8c0,5.5-4.5,10.1-10.1,10.1c-5.6,0-10.1-4.6-10.1-10.1c0-5.6,4.5-10.1,10.1-10.1C84.2,46.7,88.7,51.3,88.7,56.8z};
  }
}

\newcommand\orcidicon[1]{\href{https://orcid.org/#1}{\mbox{\scalerel*{
\begin{tikzpicture}[yscale=-1,transform shape]
\pic{orcidlogo};
\end{tikzpicture}
}{|}}}}



\usepackage{listings}
\usepackage{xcolor} % For customizing colors (optional but recommended)

% Define Python-specific settings for listings
\lstdefinestyle{python}{
    language=Python,
    basicstyle=\ttfamily\small,
    keywordstyle=\color{blue}\bfseries,
    commentstyle=\color{green!50!black}\itshape,
    stringstyle=\color{red},
    showstringspaces=false,
    frame=single,
    numbers=left,
    numberstyle=\tiny\color{gray},
    stepnumber=1,
    numbersep=5pt,
    breaklines=true,
    breakatwhitespace=true,
    tabsize=4,
    captionpos=b
}

% Default style for listings
\lstset{style=python}

\usepackage[hidelinks, bookmarksnumbered=true]{hyperref}



